Approximate Maximum a Posteriori Carrier Phase Estimator for Wiener Phase Noise Channels using Belief Propagation

The blind phase search (BPS) algorithm for carrier phase estimation is known to have sub-optimal performance for probabilistically shaped constellations. We present a belief propagation based approximate maximum a posteriori carrier phase estimator and compare its performance with the standard and an improved BPS algorithm.

==> preamble.tex <==
\usepackage[acronym]{glossaries}
\usepackage{bm}
\usepackage{siunitx}
\usepackage{upgreek}
\usepackage{xfrac}
\usepackage{kitcolors}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{calc}
\usepackage[final=true,breaklinks=true]{hyperref}
\usepackage[normalem]{ulem}
\makeatletter
\let\MYcaption\@makecaption
\makeatother

\usepackage[font=footnotesize]{subcaption}

\makeatletter
\let\@makecaption\MYcaption
\makeatother

%\usepackage{orcidlink}
\usepackage{mleftright}
\usepackage{booktabs}
%\usepackage{todonotes}
\usepackage[noadjust]{cite}


% Define names of \autoref. \Autoref (capital 'A') is used for the beginning of a sentence (where the ref names like Fig. are typically not abbreviated).
\newif\ifautorefabbr
\autorefabbrtrue
% Figure
\renewcommand*{\figureautorefname}{\ifautorefabbr Fig.\else Figure \fi}
% Chapter
\renewcommand*{\chapterautorefname}{\ifautorefabbr Chapter\else Chapter \fi}
% ((Sub)sub)section
\renewcommand*{\sectionautorefname}{\ifautorefabbr Sec.\else Section \fi}
%\renewcommand*{\subsectionautorefname}{\ifautorefabbr Sec.\@ \else Section \fi}
%\renewcommand*{\subsubsectionautorefname}{\ifautorefabbr Sec.\@ \else Section \fi}
% \renewcommand*{\equationautorefname}{(#2\null)
\providecommand*{\algorithmautorefname}{\ifautorefabbr Alg.\@ \else Algorithm \fi}
% Task
%\renewcommand*{\itemautorefname}{\ifautorefabbr Task\@ \else Task \fi}


\pgfplotsset{
  discard if/.style 2 args={
    x filter/.code={
      \edef\tempa{\thisrow{#1}}
      \edef\tempb{#2}
      \ifx\tempa\tempb
      \def\pgfmathresult{inf}
      \fi
    }
  },
  discard if not/.style 2 args={
    x filter/.code={
      \edef\tempa{\thisrow{#1}}
      \edef\tempb{#2}
      \ifx\tempa\tempb
      \else
      \def\pgfmathresult{inf}
      \fi
    }
  }
}

\let\Re\relax
\let\Im\relax
\DeclareMathOperator{\Re}{Re}
\DeclareMathOperator{\Im}{Im}
\DeclareMathOperator{\e}{e}
\let\j\relax
\DeclareMathOperator{\j}{j}
\DeclareMathOperator{\T}{T}
\definecolor{cb-1}{HTML}{4477AA}
\definecolor{cb-2}{HTML}{EE6677}
\definecolor{cb-3}{HTML}{228833}
\definecolor{cb-4}{HTML}{CCBB44}
\definecolor{cb-5}{HTML}{66CCEE}
\definecolor{cb-6}{HTML}{AA3377}
\definecolor{cb-7}{HTML}{BBBBBB}


\pgfplotscreateplotcyclelist{cb list}{
    cb-1,cb-2,cb-3,cb-4,cb-5,cb-6,cb-7
}


%\input{acronyms.tex}

\colorlet{KITColor1}{kit-blue100}
\colorlet{KITColor2}{kit-orange100}
\colorlet{KITColor3}{kit-purple100}
\colorlet{KITColor4}{kit-maigreen100}
\colorlet{KITColor5}{kit-cyanblue100}
% Some very useful LaTeX packages include:
% (uncomment the ones you want to load)
\sisetup{
  per-mode=fraction,
  fraction-function=\sfrac
}
\DeclareSIUnit\bit{bit}
\DeclareSIUnit\symbol{symbol}
\usetikzlibrary{fit, positioning, calc, angles, arrows.meta, bending, backgrounds}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{pgfplots.groupplots}
\pgfplotsset{compat=1.17}

\usepackage{algorithm}
\usepackage{algpseudocode}

\algblockdefx{cIf}{cEndIf}
[1]{\tikzmk{A}\vspace*{1ex}\textbf{if} #1 \textbf{then}}
[2][0.95]{\tikzmk{B}\textbf{end if}\vspace*{1ex}\boxit[#1]{#2}}
\algcblock[cbox]{cIf}{Else}{cEndIf}
\algrenewcommand{\algorithmiccomment}[2][.47]{\hfill\normalsize$\triangleright$ \parbox[t]{#1\linewidth}{#2}}

% define a marking command
\newcommand*{\tikzmk}[1]{\tikz[remember picture,overlay,] \node (#1) {};\ignorespaces}
% define a boxing command, argument = colour of box
\newcommand{\boxit}[2][.95]{\tikz[remember picture,overlay]{\node[yshift=1ex,fill=#2,opacity=.25,fit={(A)($(B)+(#1\linewidth,-2ex)$)}] {};}\ignorespaces}

\makeatletter
\DeclareRobustCommand{\rvdots}{%
  \vbox{
    \baselineskip4\p@\lineskiplimit\z@
    \kern-\p@
    \hbox{.}\hbox{.}\hbox{.}
  }}
\makeatother



% Makros
\pgfplotsset{colormap/blackwhite}
\pgfplotsset{colormap/bluered}
\pgfplotsset{colormap={kit-cm}{color={KITblue} color={KITorange}}}

\newcommand{\plotdecisionregion}[4]{
  \begin{tikzpicture}%[scale=0.52]
  \pgfplotsset{compat=newest}
    \begin{axis}[
      xlabel={$\Re\left\{\hat{x}_k\right\}$},
      ylabel={$\Im\left\{\hat{x}_k\right\}$},
      height=0.6\columnwidth,
      width=0.6\columnwidth,
      ylabel near ticks,
      % xlabel near ticks,
      xmin=-2,
      xmax=2,
      ymin=-2,
      ymax=2,
      grid=none,
      label style={font=\footnotesize},
      tick label style={font=\footnotesize},
      view={0}{90},
      unbounded coords=jump,
      point meta rel=per plot,
      ]
      \addplot3
      [surf,
       shader=flat,
 %     mesh/ordering=y varies,
       mesh/cols=50,
       point meta min=-5,
       point meta max=5,
       ]
      table [col sep=tab, x=real, y=imag, z=LLR]
      {#1#3.txt};
    \addplot[
      scatter,
      scatter/use mapped color={
        draw=mapped color,
        fill=mapped color,
      },
      % only marks,
      mark=*,
      mark size=1.7pt,
      draw=none,
      colormap name=blackwhite,
      point meta=explicit,
      point meta min=0,
      point meta max=1,
      ]
      table[col sep=tab, meta=bit#3]
      {#2};
    \end{axis}
    \node[below = 3mm,xshift=-0.7cm] {\footnotesize #4)};
     \end{tikzpicture}
}
\newsavebox\neuralnetwork
\sbox{\neuralnetwork}{%
		\begin{tikzpicture}[
      >=stealth,
      scale=.9,
      every node/.append style={transform shape},
      remember picture,
      ]%[>=latex']
      \tikzset{Source1b/.style={rectangle, draw=black, thick, minimum width=0.05cm, minimum height=1.2cm, rounded corners=0.5mm}}
      \tikzset{Source3/.style={rectangle, draw, thick, minimum width=0.6cm, minimum height=0.45cm, rounded corners=0.5mm}}

      \tikzset{OnehotNode/.style={circle, thick, draw,minimum width=0.1cm}}
      \tikzset{ReLUNode/.style={circle,thick,draw,fill=black!10!white}}
      \tikzset{MZMNode/.style={circle,thick,draw,fill=black!30!white}}
      % \tikzset{SoftmaxNode/.style={circle,thick,draw,fill=black!60!white}}
   % \node [Source1b, minimum height=12cm] (serial) at (3.6,0) {}; %[rotate=90] {Seralizer};
   \node (serial) at (3.6,0) {};
   % \node [rotate=-90,anchor=south west] at (serial.north east) {Serializer};
	  \def\offseta{4.5}
	  \def\offsetb{0.5cm}
	  \def\offsetc{15cm}
    \def\k{0}
    \def\ki{1}
        \node [OnehotNode] (S\ki1) at ($(0,0.5)+(0,\k)$) {};
        \node [OnehotNode] (S\ki2) at ($(0,-0.5)+(0,\k)$) {};
		\node at ($(0,0)+(0,\k)$) {$\rvdots$};
		\draw [->] ($(S\ki1)+(-0.4cm,0)$) -- (S\ki1);
		\draw [->] ($(S\ki2)+(-0.4cm,0)$) -- (S\ki2);
		% \node [rotate=90,anchor=south] at ($(0,0)+(-0.4cm,\k)$) {one-hot vector};

		\node [ReLUNode] (H\ki11) at ($(1,1.5)+(0,\k)$) {};
		\node [ReLUNode] (H\ki12) at ($(1,0.5)+(0,\k)$) {};
		\node [ReLUNode] (H\ki13) at ($(1,-0.5)+(0,\k)$) {};
		\node [ReLUNode] (H\ki14) at ($(1,-1.5)+(0,\k)$) {};
		\node at ($(1,0)+(0,\k)$) [anchor=center] {$\rvdots$};

		\foreach\j in {1,2,3,4}{
		  \draw [->] (S\ki1) -- (H\ki1\j); \draw [->] (S\ki2) -- (H\ki1\j);
		};

		\node [ReLUNode] (H\ki21) at ($(2,1.5)+(0,\k)$) {};
		\node [ReLUNode] (H\ki22) at ($(2,0.5)+(0,\k)$) {};
		\node [ReLUNode] (H\ki23) at ($(2,-0.5)+(0,\k)$) {};
		\node [ReLUNode] (H\ki24) at ($(2,-1.5)+(0,\k)$) {};
		\node at ($(2,0)+(0,\k)$) [anchor=center] {$\rvdots$};

		\foreach\j in {1,2,3,4}{
		  \foreach\i in {1,2,3,4}{
		    \draw [->] (H\ki1\j) -- (H\ki2\i);
		  };
		};


		\node [MZMNode] (M\ki1) at ($(3,1)+(0,\k)$) {};
		\node [MZMNode] (M\ki2) at ($(3,0)+(0,\k)$) {};
		\node [MZMNode] (M\ki3) at ($(3,-1)+(0,\k)$) {};
		\draw [<-] ($(serial.west)+(0,\k)+(0,1)$) -- (M\ki1.east);
		\draw [<-] ($(serial.west)+(0,\k)$) -- (M\ki2.east);
		\draw [<-] ($(serial.west)+(0,\k)+(0,-1)$) -- (M\ki3.east);

		\node at ($(3,-0.5)+(0,\k)$) [anchor=center] {$\rvdots$};
		\node at ($(3,+0.5)+(0,\k)$) [anchor=center] {$\rvdots$};
		\foreach\j in {1,2,3,4}{
		  \foreach\i in {1,2,3}{
		    \draw [->] (H\ki2\j) -- (M\ki\i);
		  };
		};
\end{tikzpicture}%
}

%%% Paper Review commands

\definecolor{cR0}{RGB}{0, 0, 255} % blau
\definecolor{cR1}{RGB}{140,182,60} % maigrün
\definecolor{cR2}{RGB}{162,34,35} % rot
\definecolor{cR3}{RGB}{35,161,224} % cyan

\definecolor{cR12}{RGB}{223,155,27} % orange
\definecolor{cR13}{RGB}{0,150,130} % teal
\definecolor{cR23}{RGB}{163,16,124} % purple

\definecolor{cR123}{RGB}{167,130,46} % brown
\definecolor{cR03}{RGB}{255, 0, 187} % pink

\newcommand{\RevI}[1]{#1}
\newcommand{\RevII}[1]{#1}
\newcommand{\RevIII}[1]{#1}

